Limited-Angle Tomography Reconstruction via Deep End-To-End Learning on Synthetic Data

Computed tomography (CT) has become an essential part of modern science and medicine. A CT scanner consists of an X-ray source that is spun around an object of interest. On the opposite end of the X-ray source, a detector captures X-rays that are not absorbed by the object. The reconstruction of an image is a linear inverse problem, which is usually solved by filtered back projection. However, when the number of measurements is small, the reconstruction problem is ill-posed. This is for example the case when the X-ray source is not spun completely around the object, but rather irradiates the object only from a limited angle. To tackle this problem, we present a deep neural network that is trained on a large amount of carefully-crafted synthetic data and can perform limited-angle tomography reconstruction even for only 30{\deg} or 40{\deg} sinograms. With our approach we won the first place in the Helsinki Tomography Challenge 2022.

==> figures/generated/no_voronoi.tex <==
\node at (0, 0) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/000.png}};
\node at (1, 0) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/001.png}};
\node at (2, 0) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/002.png}};
\node at (3, 0) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/003.png}};
\node at (4, 0) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/004.png}};
\node at (0, 1) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/005.png}};
\node at (1, 1) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/006.png}};
\node at (2, 1) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/007.png}};
\node at (3, 1) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/008.png}};
\node at (4, 1) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/009.png}};
\node at (0, 2) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/010.png}};
\node at (1, 2) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/011.png}};
\node at (2, 2) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/012.png}};
\node at (3, 2) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/013.png}};
\node at (4, 2) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/014.png}};
\node at (0, 3) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/015.png}};
\node at (1, 3) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/016.png}};
\node at (2, 3) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/017.png}};
\node at (3, 3) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/018.png}};
\node at (4, 3) {\includegraphics[width=\imgwidth]{figures/generated/no_voronoi/019.png}};


==> figures/generated/voronoi.tex <==
\node at (0, 0) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/000.png}};
\node at (1, 0) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/001.png}};
\node at (2, 0) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/002.png}};
\node at (3, 0) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/003.png}};
\node at (4, 0) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/004.png}};
\node at (0, 1) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/005.png}};
\node at (1, 1) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/006.png}};
\node at (2, 1) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/007.png}};
\node at (3, 1) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/008.png}};
\node at (4, 1) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/009.png}};
\node at (0, 2) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/010.png}};
\node at (1, 2) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/011.png}};
\node at (2, 2) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/012.png}};
\node at (3, 2) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/013.png}};
\node at (4, 2) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/014.png}};
\node at (0, 3) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/015.png}};
\node at (1, 3) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/016.png}};
\node at (2, 3) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/017.png}};
\node at (3, 3) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/018.png}};
\node at (4, 3) {\includegraphics[width=\imgwidth]{figures/generated/voronoi/019.png}};

